Simultaneous observations of a breakout current sheet and a flare current sheet in a coronal jet event

Previous studies have revealed that solar coronal jets triggered by the eruption of mini-filaments (MFs) conform to the famous magnetic-breakout mechanism. In such scenario, a breakout current sheet (BCS) and a flare current sheet (FCS) should be observed during the jets. With high spatial and temporal resolution data from the SDO, the NVST, the RHESSI, the Wind, and the GOES, we present observational evidence of a BCS and a FCS formation during coronal jets driven by a MF eruption occurring in the active region NOAA 11726 on 2013 April 21. Magnetic field extrapolation show that the MF was enclosed by a fan-spine magnetic structure. The MF was activated by flux cancellation under it, and then slowly rose. A BCS formed when the magnetic fields wrapping the MF squeezed to antidirectional external open fields. Simultaneously, one thin bright jet and two bidirectional jet-like structures were observed. As the MF erupted as a blowout jet, a FCS was formed when the two distended legs inside the MF field came together. One end of the FCS connected the post-flare loops. The peak temperature of BCS was calculated to be 2.5 MK. The length, width and peak temperature of FCS was calculated to be 4.35-4.93 Mm, 1.31-1.45 Mm, and 2.5 MK, respectively. The magnetic reconnection rate associated with the FCS was estimated to be from 0.266 to 0.333. This event also related to a type III radio burst, indicating its influence on interplanetary space. These observations support the scenario of the breakout model as the trigger mechanism of coronal jets, and flux cancellation was the driver of this event.

==> arxiv-2206.13080 <==
<?xml version="1.0" encoding="UTF-8"?>
<!DOCTYPE html PUBLIC "-//W3C//DTD XHTML 1.0 Transitional//EN" "http://www.w3.org/TR/xhtml1/DTD/xhtml1-transitional.dtd">
<html xmlns="http://www.w3.org/1999/xhtml" lang="en" xml:lang="en">

<head>  <title>[2206.13080] Plausibility of ultraviolet burst generation in the low solar chromosphere</title>
  <meta name="viewport" content="width=device-width, initial-scale=1">
  <link rel="apple-touch-icon" sizes="180x180" href="/static/browse/0.3.4/images/icons/apple-touch-icon.png">
  <link rel="icon" type="image/png" sizes="32x32" href="/static/browse/0.3.4/images/icons/favicon-32x32.png">
  <link rel="icon" type="image/png" sizes="16x16" href="/static/browse/0.3.4/images/icons/favicon-16x16.png">
  <link rel="manifest" href="/static/browse/0.3.4/images/icons/site.webmanifest">
  <link rel="mask-icon" href="/static/browse/0.3.4/images/icons/safari-pinned-tab.svg" color="#5bbad5">
  <meta name="msapplication-TileColor" content="#da532c">
  <meta name="theme-color" content="#ffffff">
  <link rel="stylesheet" type="text/css" media="screen" href="/static/browse/0.3.4/css/arXiv.css?v=20230622" />
  <link rel="stylesheet" type="text/css" media="print" href="/static/browse/0.3.4/css/arXiv-print.css?v=20200611" />
  <link rel="stylesheet" type="text/css" media="screen" href="/static/browse/0.3.4/css/browse_search.css" />
  <script language="javascript" src="/static/browse/0.3.4/js/accordion.js" /></script>
  <link rel="canonical" href="/abs/2206.13080"/><meta property="og:type" content="website" />
<meta property="og:site_name" content="arXiv.org" />
<meta property="og:title" content="Plausibility of ultraviolet burst generation in the low solar chromosphere" />
<meta property="og:url" content="https://arxiv.org/abs/2206.13080v2" />
<meta property="og:image" content="/static/browse/0.3.4/images/arxiv-logo-fb.png" />
<meta property="og:image:secure_url" content="/static/browse/0.3.4/images/arxiv-logo-fb.png" />
<meta property="og:image:width" content="1200" />
<meta property="og:image:height" content="700" />
<meta property="og:image:alt" content="arXiv logo"/>
<meta property="og:description" content="Ultraviolet (UV) bursts and Ellerman bombs (EBs) are small-scale magnetic reconnection events taking place in the highly stratified, low solar atmosphere. It is still not clear whether UV bursts have to be generated at a higher atmospheric layer than EBs or whether both UV bursts and EBs can occur in the low chromosphere. We numerically studied the low $β$ magnetic reconnection process around the solar temperature minimum region (TMR). The time-dependent ionization degrees of hydrogen and helium are included in the MHD code, which lead to a more realistic magnetic diffusion caused by electron-neutral collision and ambipolar diffusion. A more realistic radiative cooling model from Carlsson &amp; Leenaarts 2012 is included in the simulations. Our results in high resolution indicate that the plasmas in the reconnection region are heated up to more than $20,000$ K if the reconnecting magnetic field is as strong as $500$ G, which suggests that UV bursts can be generated in the dense low chromosphere. The dominant mechanism for producing the UV burst in the low chromosphere is heating, as a result of the local compression in the reconnection process. The thermal energy occurring in the reconnection region rapidly increases after the turbulent reconnection mediated by plasmoids is invoked. The average power density of the generated thermal energy in the reconnection region can reach over $1000$ erg cm$^{-3}$ s$^{-1}$, which is comparable to the average power density accounting for a UV burst. With the strength of the reconnecting magnetic field exceeding $900$ G, the width of the synthesized Si IV 1394 A line profile with multiple peaks can reach up to $100$ km s$^{-1}$, which is consistent with observations."/>
<meta name="twitter:site" content="@arxiv"/>
<meta name="twitter:card" content="summary"/>
<meta name="twitter:title" content="Plausibility of ultraviolet burst generation in the low solar chromosphere"/>
<meta name="twitter:description" content="Ultraviolet (UV) bursts and Ellerman bombs (EBs) are small-scale magnetic reconnection events taking place in the highly stratified, low solar atmosphere. It is still not clear whether UV bursts..."/>
<meta name="twitter:image" content="https://static.arxiv.org/icons/twitter/arxiv-logo-twitter-square.png"/>
<meta name="twitter:image:alt" content="arXiv logo"/>
  <link rel="stylesheet" media="screen" type="text/css" href="/static/browse/0.3.4/css/tooltip.css"/><link rel="stylesheet" media="screen" type="text/css" href="https://static.arxiv.org/js/bibex-dev/bibex.css?20200709"/>  <script src="/static/browse/0.3.4/js/mathjaxToggle.min.js" type="text/javascript"></script>  <script src="//code.jquery.com/jquery-latest.min.js" type="text/javascript"></script>
  <script src="//cdn.jsdelivr.net/npm/js-cookie@2/src/js.cookie.min.js" type="text/javascript"></script>
  <script src="//cdn.jsdelivr.net/npm/dompurify@2.3.5/dist/purify.min.js"></script>
  <script src="/static/browse/0.3.4/js/toggle-labs.js?20230622" type="text/javascript"></script>
  <script src="/static/browse/0.3.4/js/cite.js" type="text/javascript"></script><meta name="citation_title" content="Plausibility of ultraviolet burst generation in the low solar chromosphere" /><meta name="citation_author" content="Ni, Lei" /><meta name="citation_author" content="Cheng, Guanchong" /><meta name="citation_author" content="Lin, Jun" /><meta name="citation_doi" content="10.1051/0004-6361/202243304" /><meta name="citation_date" content="2022/06/27" /><meta name="citation_online_date" content="2022/07/27" /><meta name="citation_pdf_url" content="http://arxiv.org/pdf/2206.13080.pdf" /><meta name="citation_arxiv_id" content="2206.13080" /><meta name="citation_abstract" content="Ultraviolet (UV) bursts and Ellerman bombs (EBs) are small-scale magnetic reconnection events taking place in the highly stratified, low solar atmosphere. It is still not clear whether UV bursts have to be generated at a higher atmospheric layer than EBs or whether both UV bursts and EBs can occur in the low chromosphere. We numerically studied the low $\beta$ magnetic reconnection process around the solar temperature minimum region (TMR). The time-dependent ionization degrees of hydrogen and helium are included in the MHD code, which lead to a more realistic magnetic diffusion caused by electron-neutral collision and ambipolar diffusion. A more realistic radiative cooling model from Carlsson &amp; Leenaarts 2012 is included in the simulations. Our results in high resolution indicate that the plasmas in the reconnection region are heated up to more than $20,000$ K if the reconnecting magnetic field is as strong as $500$ G, which suggests that UV bursts can be generated in the dense low chromosphere. The dominant mechanism for producing the UV burst in the low chromosphere is heating, as a result of the local compression in the reconnection process. The thermal energy occurring in the reconnection region rapidly increases after the turbulent reconnection mediated by plasmoids is invoked. The average power density of the generated thermal energy in the reconnection region can reach over $1000$ erg cm$^{-3}$ s$^{-1}$, which is comparable to the average power density accounting for a UV burst. With the strength of the reconnecting magnetic field exceeding $900$ G, the width of the synthesized Si IV 1394 A line profile with multiple peaks can reach up to $100$ km s$^{-1}$, which is consistent with observations." />
</head>

<body  class="with-cu-identity">
  
  <div class="flex-wrap-footer">
    <header>
      <a href="#content" class="is-sr-only">Skip to main content</a>
      <!-- start desktop header -->
      <div class="columns is-vcentered is-hidden-mobile" id="cu-identity">
        <div class="column" id="cu-logo">
          <a href="https://www.cornell.edu/"><img src="/static/browse/0.3.4/images/icons/cu/cornell-reduced-white-SMALL.svg" alt="Cornell University" /></a>
        </div><div class="column">
            <a href="https://info.arxiv.org/help/cloud.html"><span style="color:white;text-decoration-line:underline;">
                Served from the cloud
            </span></a>
        </div><div class="column" id="support-ack">
          <span id="support-ack-url">We gratefully acknowledge support from the Simons Foundation, <a href="https://info.arxiv.org/about/ourmembers.html">member institutions</a>, and all contributors. <a href="https://info.arxiv.org/about/donate.html">Donate</a></span>
        </div>
      </div>

      <div id="header" class="is-hidden-mobile">
<a aria-hidden="true" href="{url_path('ignore_me')}"></a>
  <div class="header-breadcrumbs is-hidden-mobile">
    <a href="/"><img src="/static/browse/0.3.4/images/arxiv-logo-one-color-white.svg" alt="arxiv logo" style="height:40px;"/></a> <span>&gt;</span> <a href="/list/astro-ph/recent">astro-ph</a> <span>&gt;</span> arXiv:2206.13080
  </div>
          <div class="search-block level-right">
    <form class="level-item mini-search" method="GET" action="https://arxiv.org/search">
      <div class="field has-addons">
        <div class="control">
          <input class="input is-small" type="text" name="query" placeholder="Search..." aria-label="Search term or terms" />
          <p class="help"><a href="https://info.arxiv.org/help">Help</a> | <a href="https://arxiv.org/search/advanced">Advanced Search</a></p>
        </div>
        <div class="control">
          <div class="select is-small">
            <select name="searchtype" aria-label="Field to search">
              <option value="all" selected="selected">All fields</option>
              <option value="title">Title</option>
              <option value="author">Author</option>
              <option value="abstract">Abstract</option>
              <option value="comments">Comments</option>
              <option value="journal_ref">Journal reference</option>
              <option value="acm_class">ACM classification</option>
              <option value="msc_class">MSC classification</option>
              <option value="report_num">Report number</option>
              <option value="paper_id">arXiv identifier</option>
              <option value="doi">DOI</option>
              <option value="orcid">ORCID</option>
              <option value="author_id">arXiv author ID</option>
              <option value="help">Help pages</option>
              <option value="full_text">Full text</option>
            </select>
          </div>
        </div>
        <input type="hidden" name="source" value="header">
        <button class="button is-small is-cul-darker">Search</button>
      </div>
    </form>
  </div>
     </div><!-- /end desktop header -->

      <div class="mobile-header">
        <div class="columns is-mobile">
          <div class="column logo-arxiv"><a href="https://arxiv.org/"><img src="/static/browse/0.3.4/images/arxiv-logomark-small-white.svg" alt="arXiv logo" style="height:60px;" /></a></div>
          <div class="column logo-cornell"><a href="https://www.cornell.edu/">
            <picture>
              <source media="(min-width: 501px)"
                srcset="/static/browse/0.3.4/images/icons/cu/cornell-reduced-white-SMALL.svg  400w"
                sizes="400w" />
              <source srcset="/static/browse/0.3.4/images/icons/cu/cornell_seal_simple_black.svg 2x" />
              <img src="/static/browse/0.3.4/images/icons/cu/cornell-reduced-white-SMALL.svg" alt="Cornell University Logo" />
            </picture>
          </a></div>
          <div class="column nav" id="toggle-container" role="menubar">
            <button class="toggle-control"><svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 512 512" class="icon filter-white"><title>open search</title><path d="M505 442.7L405.3 343c-4.5-4.5-10.6-7-17-7H372c27.6-35.3 44-79.7 44-128C416 93.1 322.9 0 208 0S0 93.1 0 208s93.1 208 208 208c48.3 0 92.7-16.4 128-44v16.3c0 6.4 2.5 12.5 7 17l99.7 99.7c9.4 9.4 24.6 9.4 33.9 0l28.3-28.3c9.4-9.4 9.4-24.6.1-34zM208 336c-70.7 0-128-57.2-128-128 0-70.7 57.2-128 128-128 70.7 0 128 57.2 128 128 0 70.7-57.2 128-128 128z"/></svg></button>
            <div class="mobile-toggle-block toggle-target">
              <form class="mobile-search-form" method="GET" action="https://arxiv.org/search">
                <div class="field has-addons">
                  <input class="input" type="text" name="query" placeholder="Search..." aria-label="Search term or terms" />
                  <input type="hidden" name="source" value="header">
                  <input type="hidden" name="searchtype" value="all">
                  <button class="button">GO</button>
                </div>
              </form>
            </div>

            <button class="toggle-control"><svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 448 512" class="icon filter-white" role="menu"><title>open navigation menu</title><path d="M16 132h416c8.837 0 16-7.163 16-16V76c0-8.837-7.163-16-16-16H16C7.163 60 0 67.163 0 76v40c0 8.837 7.163 16 16 16zm0 160h416c8.837 0 16-7.163 16-16v-40c0-8.837-7.163-16-16-16H16c-8.837 0-16 7.163-16 16v40c0 8.837 7.163 16 16 16zm0 160h416c8.837 0 16-7.163 16-16v-40c0-8.837-7.163-16-16-16H16c-8.837 0-16 7.163-16 16v40c0 8.837 7.163 16 16 16z"/ ></svg></button>
            <div class="mobile-toggle-block toggle-target">
              <nav class="mobile-menu" aria-labelledby="mobilemenulabel">
                <h2 id="mobilemenulabel">quick links</h2>
                <ul>
                    <li><a href="https://arxiv.org/login">Login</a></li>
                    <li><a href="https://info.arxiv.org/help">Help Pages</a></li>
                    <li><a href="https://info.arxiv.org/about">About</a></li>
                </ul>
              </nav>
            </div>
          </div>
        </div>
      </div><!-- /end mobile-header -->
    </header>

    <main>
      <div id="content">
<!--
rdf:RDF xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#"
         xmlns:dc="http://purl.org/dc/elements/1.1/"
         xmlns:trackback="http://madskills.com/public/xml/rss/module/trackback/">
    <rdf:Description
        rdf:about="/abs/2206.13080"
        dc:identifier="/abs/2206.13080"
        dc:title="Plausibility of ultraviolet burst generation in the low solar chromosphere"
        trackback:ping="/trackback/2206.13080" />
    </rdf:RDF>
--><div id="abs-outer">

  <div class="leftcolumn">
    <div class="subheader">
      <h1>Astrophysics > Solar and Stellar Astrophysics</h1>
    </div>

    <div class="header-breadcrumbs-mobile">
      <strong>arXiv:2206.13080</strong> (astro-ph)
    </div>
<link rel="stylesheet" type="text/css" href="/static/base/1.0.1/css/abs.css">
<div id="content-inner">
  <div id="abs">
    <div class="dateline">
  [Submitted on 27 Jun 2022 (<a href="https://arxiv.org/abs/2206.13080v1">v1</a>), last revised 27 Jul 2022 (this version, v2)]</div>
    <h1 class="title mathjax"><span class="descriptor">Title:</span>Plausibility of ultraviolet burst generation in the low solar chromosphere</h1>
    <div class="authors"><span class="descriptor">Authors:</span><a href="https://arxiv.org/search/astro-ph?searchtype=author&amp;query=Ni,+L">Lei Ni</a>, <a href="https://arxiv.org/search/astro-ph?searchtype=author&amp;query=Cheng,+G">Guanchong Cheng</a>, <a href="https://arxiv.org/search/astro-ph?searchtype=author&amp;query=Lin,+J">Jun Lin</a></div>            <div id="download-button-info" hidden>Download a PDF of the paper titled Plausibility of ultraviolet burst generation in the low solar chromosphere, by Lei Ni and 2 other authors</div>
    <a class="mobile-submission-download" href="/pdf/2206.13080.pdf">Download PDF</a>



    <blockquote class="abstract mathjax">
            <span class="descriptor">Abstract:</span>Ultraviolet (UV) bursts and Ellerman bombs (EBs) are small-scale magnetic reconnection events taking place in the highly stratified, low solar atmosphere. It is still not clear whether UV bursts have to be generated at a higher atmospheric layer than EBs or whether both UV bursts and EBs can occur in the low chromosphere. We numerically studied the low $\beta$ magnetic reconnection process around the solar temperature minimum region (TMR). The time-dependent ionization degrees of hydrogen and helium are included in the MHD code, which lead to a more realistic magnetic diffusion caused by electron-neutral collision and ambipolar diffusion. A more realistic radiative cooling model from Carlsson &amp; Leenaarts 2012 is included in the simulations. Our results in high resolution indicate that the plasmas in the reconnection region are heated up to more than $20,000$ K if the reconnecting magnetic field is as strong as $500$ G, which suggests that UV bursts can be generated in the dense low chromosphere. The dominant mechanism for producing the UV burst in the low chromosphere is heating, as a result of the local compression in the reconnection process. The thermal energy occurring in the reconnection region rapidly increases after the turbulent reconnection mediated by plasmoids is invoked. The average power density of the generated thermal energy in the reconnection region can reach over $1000$ erg cm$^{-3}$ s$^{-1}$, which is comparable to the average power density accounting for a UV burst. With the strength of the reconnecting magnetic field exceeding $900$ G, the width of the synthesized Si IV 1394 A line profile with multiple peaks can reach up to $100$ km s$^{-1}$, which is consistent with observations.
    </blockquote>

    <!--CONTEXT-->
    <div class="metatable">
      <table summary="Additional metadata">        <tr>
          <td class="tablecell label">Comments:</td>
          <td class="tablecell comments mathjax">12 pages, 10 figures</td>
        </tr>
<tr>
          <td class="tablecell label">Subjects:</td>
          <td class="tablecell subjects">
            <span class="primary-subject">Solar and Stellar Astrophysics (astro-ph.SR)</span>; Plasma Physics (physics.plasm-ph); Space Physics (physics.space-ph)</td>
        </tr><tr>
          <td class="tablecell label">Cite as:</td>
          <td class="tablecell arxivid"><span class="arxivid"><a href="https://arxiv.org/abs/2206.13080">arXiv:2206.13080</a> [astro-ph.SR]</span></td>
        </tr>
        <tr>
          <td class="tablecell label">&nbsp;</td>
          <td class="tablecell arxividv">(or <span class="arxivid">
              <a href="https://arxiv.org/abs/2206.13080v2">arXiv:2206.13080v2</a> [astro-ph.SR]</span> for this version)
          </td>
        </tr>        <tr>
          <td class="tablecell label">&nbsp;</td>
          <td class="tablecell arxivdoi">
            <a href="https://doi.org/10.48550/arXiv.2206.13080">https://doi.org/10.48550/arXiv.2206.13080</a>
            <div class="button-and-tooltip">
              <button class="more-info" aria-describedby="more-info-desc-1">
                <svg height="15" role="presentation" xmlns="http://www.w3.org/2000/svg" viewBox="0 0 512 512"><path fill="currentColor" d="M256 8C119.043 8 8 119.083 8 256c0 136.997 111.043 248 248 248s248-111.003 248-248C504 119.083 392.957 8 256 8zm0 110c23.196 0 42 18.804 42 42s-18.804 42-42 42-42-18.804-42-42 18.804-42 42-42zm56 254c0 6.627-5.373 12-12 12h-88c-6.627 0-12-5.373-12-12v-24c0-6.627 5.373-12 12-12h12v-64h-12c-6.627 0-12-5.373-12-12v-24c0-6.627 5.373-12 12-12h64c6.627 0 12 5.373 12 12v100h12c6.627 0 12 5.373 12 12v24z" class=""></path></svg>
                <span class="visually-hidden">Focus to learn more</span>
              </button>
              <!-- tooltip description -->
              <div role="tooltip" id="more-info-desc-1">
                <span class="left-corner"></span>
                arXiv-issued DOI via DataCite
              </div>
            </div>
          </td>
        </tr>        <tr>
          <td class="tablecell label">Journal&nbsp;reference:</td>
          <td class="tablecell jref">A&amp;A 665, A116 (2022)</td>
        </tr>
        <tr>
          <td class="tablecell label">
            <abbr title="Digital Object Identifier">Related DOI</abbr>:
          </td>
          <td class="tablecell doi"><a href="https://doi.org/10.1051/0004-6361/202243304" data-doi="10.1051/0004-6361/202243304" class="link-https link-external" rel="external noopener nofollow">https://doi.org/10.1051/0004-6361/202243304</a>

            <!-- accessible tooltip example -->
            <div class="button-and-tooltip">
              <button class="more-info" aria-describedby="more-info-desc-1">
                <svg height="15" role="presentation" xmlns="http://www.w3.org/2000/svg" viewBox="0 0 512 512"><path fill="currentColor" d="M256 8C119.043 8 8 119.083 8 256c0 136.997 111.043 248 248 248s248-111.003 248-248C504 119.083 392.957 8 256 8zm0 110c23.196 0 42 18.804 42 42s-18.804 42-42 42-42-18.804-42-42 18.804-42 42-42zm56 254c0 6.627-5.373 12-12 12h-88c-6.627 0-12-5.373-12-12v-24c0-6.627 5.373-12 12-12h12v-64h-12c-6.627 0-12-5.373-12-12v-24c0-6.627 5.373-12 12-12h64c6.627 0 12 5.373 12 12v100h12c6.627 0 12 5.373 12 12v24z" class=""></path></svg>
                <span class="visually-hidden">Focus to learn more</span>
              </button>
              <!-- tooltip description -->
              <div role="tooltip" id="more-info-desc-1">
                <span class="left-corner"></span>
                DOI(s) linking to related resources
              </div>
            </div>
          </td>
        </tr>
</table>
    </div>
  </div>
</div>
    <div class="submission-history">
      <h2>Submission history</h2> From: Lei Ni [<a href="/show-email/c5534682/2206.13080">view email</a>]      <br/>            <strong><a href="/abs/2206.13080v1">[v1]</a></strong>
        Mon, 27 Jun 2022 06:54:20 UTC (23,686 KB)<br/>
    <strong>[v2]</strong>
        Wed, 27 Jul 2022 08:15:42 UTC (23,684 KB)<br/>
</div>
  </div>
  <!--end leftcolumn-->
<div class="extra-services">    <div class="full-text">
      <a name="other"></a>
      <span class="descriptor">Full-text links:</span>
      <h2>Access Paper:</h2>
      <ul>
  <div id="download-button-info" hidden>
Download a PDF of the paper titled Plausibility of ultraviolet burst generation in the low solar chromosphere, by Lei Ni and 2 other authors</div><li><a href="/pdf/2206.13080.pdf" aria-describedby="download-button-info" accesskey="f" class="abs-button download-pdf">Download PDF</a></li><li><a href="/ps/2206.13080" class="abs-button download-ps">PostScript</a></li><li><a href="/format/2206.13080" class="abs-button download-format">Other Formats</a></li></ul>
      <div class="abs-license">(<a href="http://arxiv.org/licenses/nonexclusive-distrib/1.0/" title="Rights to this article">view license</a>)</div>
    </div>
    <!--end full-text-->    <div class="browse">
    Current browse context: <div class="current">astro-ph.SR</div>

  <div class="prevnext">
<span class="arrow">
      <a class="abs-button prev-url" href="/prevnext?id=2206.13080&amp;function=prev&amp;context=astro-ph.SR"
         accesskey="p" title="previous in astro-ph.SR (accesskey p)">&lt;&nbsp;prev</a>
    </span>
    <span class="is-hidden-mobile">&nbsp; | &nbsp;</span>    <span class="arrow">
      <a class="abs-button next-url" href="/prevnext?id=2206.13080&amp;function=next&amp;context=astro-ph.SR" accesskey="n"
         title="next in astro-ph.SR (accesskey n)">next&nbsp;&gt;</a>
    </span><br/>
  </div><div class="list">
    <a class="abs-button abs-button-grey abs-button-small context-new" href="/list/astro-ph.SR/new">new</a>
    <span class="is-hidden-mobile"> | </span>
    <a class="abs-button abs-button-grey abs-button-small context-recent" href="/list/astro-ph.SR/recent">recent</a>
    <span class="is-hidden-mobile"> | </span>
    <a class="abs-button abs-button-grey abs-button-small context-id" href="/list/astro-ph.SR/2206">2206</a>
  </div><div class="abs-switch-cat">
    Change to browse by:
    <div class="switch context-change">
        <a href="/abs/2206.13080?context=astro-ph">astro-ph</a><br class="is-hidden-mobile">
        <a href="/abs/2206.13080?context=physics">physics</a><br class="is-hidden-mobile">
        <a class="subclass" href="/abs/2206.13080?context=physics.plasm-ph">physics.plasm-ph</a><br class="is-hidden-mobile">
        <a class="subclass" href="/abs/2206.13080?context=physics.space-ph">physics.space-ph</a><br class="is-hidden-mobile">
    </div>
  </div>

    </div>

    <div class="extra-ref-cite">
      <h3>References &amp; Citations</h3>
      <ul>
        <li><a  class="abs-button abs-button-small cite-ads" href="https://ui.adsabs.harvard.edu/abs/arXiv:2206.13080">NASA ADS</a></li><li><a  class="abs-button abs-button-small cite-google-scholar" href="https://scholar.google.com/scholar_lookup?arxiv_id=2206.13080" target="_blank" rel="noopener">Google Scholar</a></li>
        <li><a  class="abs-button abs-button-small cite-semantic-scholar" href="https://api.semanticscholar.org/arXiv:2206.13080" target="_blank" rel="noopener">Semantic Scholar</a></li>
      </ul>
      <div style="clear:both;"></div>
    </div>

<div class='extra-ref-cite'>
    <a id='bib-cite-css' hidden='true' href='/static/browse/0.3.4/css/cite.css'>a</a>

    <span id='bib-cite-trigger' class="bib-cite-button abs-button">export BibTeX citation</span>
    <span id='bib-cite-loading' hidden='true'>Loading...</span>
</div>

<div id='bib-cite-modal' class='bib-modal' hidden='true'>
    <div class='bib-modal-content'>
        <div class='bib-modal-title'>
            <h2>BibTeX formatted citation</h2>
            <span class='bib-modal-close' >&times;</span>
        </div>
        <div>
            <textarea id='bib-cite-target' class="bib-citation-content" aria-label="loading the citation">loading...</textarea>
        </div>
        <div>
            <span>Data provided by: </span>
            <a id='bib-cite-source-api'></a>
        </div>
    </div>
</div><div class="bookmarks">
  <div><h3>Bookmark</h3></div><a class="abs-button abs-button-grey abs-button-small" href="https://arxiv.org/ct?url=http://www.bibsonomy.org/BibtexHandler?requTask%3Dupload%26url%3Dhttps://arxiv.org/abs/2206.13080%26description%3DPlausibility+of+ultraviolet+burst+generation+in+the+low+solar+chromosphere&amp;v=686e4287"
     title="Bookmark on BibSonomy">
    <img src="/static/browse/0.3.4/images/icons/social/bibsonomy.png"
         alt="BibSonomy logo"/>
  </a>
  <a class="abs-button abs-button-grey abs-button-small" href="https://arxiv.org/ct?url=https://reddit.com/submit?url%3Dhttps://arxiv.org/abs/2206.13080%26title%3DPlausibility+of+ultraviolet+burst+generation+in+the+low+solar+chromosphere&amp;v=d1dbebf9"
     title="Bookmark on Reddit">
    <img src="/static/browse/0.3.4/images/icons/social/reddit.png"
         alt="Reddit logo"/>
  </a>
</div>  </div>
  <!--end extra-services-->
<!-- LABS AREA -->
<div id="labstabs">
  <div class="labstabs"><input type="radio" name="tabs" id="tabone"checked="checked">
    <label for="tabone">Bibliographic Tools</label>
    <div class="tab labs-display-bib">
      <h1>Bibliographic and Citation Tools</h1>
      <div class="toggle">
        <div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input id="bibex-toggle" type="checkbox" class="lab-toggle">
              <span class="slider"></span>
              <span class="is-sr-only">Bibliographic Explorer Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-bibex">Bibliographic Explorer</span> <em>(<a href="https://info.arxiv.org/labs/showcase.html#arxiv-bibliographic-explorer">What is the Explorer?</a>)</em>
          </div>
        </div>
<div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input
                id="litmaps-toggle"
                type="checkbox"
                class="lab-toggle"
                data-script-url="/static/browse/0.3.4/js/litmaps.js?20210617"
                aria-labelledby="label-for-litmaps">
              <span class="slider"></span>
              <span class="is-sr-only">Litmaps Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-litmaps">Litmaps</span> <em>(<a href="https://www.litmaps.co/" target="_blank">What is Litmaps?</a>)</em>
          </div>
        </div>
        <div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input
                id="scite-toggle"
                type="checkbox"
                class="lab-toggle"
                data-script-url="/static/browse/0.3.4/js/scite.js?20210617"
                aria-labelledby="label-for-scite">
              <span class="slider"></span>
              <span class="is-sr-only">scite.ai Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-scite">scite Smart Citations</span> <em>(<a href="https://www.scite.ai/" target="_blank">What are Smart Citations?</a>)</em>
          </div>
        </div>
      </div>
        <div class="labs-content-placeholder labs-display" style="display: none;"></div>
        <div style="min-height: 15px" id="litmaps-open-in"></div>
        <div style="min-height: 15px" id="scite-open-in"></div>
    </div>


    <input type="radio" name="tabs" id="tabtwo">
    <label for="tabtwo">Code, Data, Media</label>
    <div class="tab">
      <h1>Code, Data and Media Associated with this Article</h1>
      <div class="toggle">
        <div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input        
                id="catalyzex-toggle"
                data-script-url="/static/browse/0.3.4/js/catalyzex.js"
                type="checkbox" class="lab-toggle" aria-labelledby="label-for-cx">
              <span class="slider"></span>
              <span class="is-sr-only">Links to Code Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-cx">CatalyzeX Code Finder for Papers</span> <em>(<a href="https://www.catalyzex.com" target="_blank">What is CatalyzeX?</a>)</em>
          </div>
        </div>

        <div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input
                id="dagshub-toggle"
                data-script-url="/static/browse/0.3.4/js/dagshub.js"
                type="checkbox" class="lab-toggle" aria-labelledby="label-for-dagshub">
              <span class="slider"></span>
              <span class="is-sr-only">DagsHub Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-dagshub">DagsHub</span> <em>(<a href="https://dagshub.com/" target="_blank">What is DagsHub?</a>)</em>
          </div>
        </div>
  
        <div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input
                id="paperwithcode-toggle"
                data-script-url="/static/browse/0.3.4/js/paperswithcode.js"
                type="checkbox" class="lab-toggle" aria-labelledby="label-for-pwc">
              <span class="slider"></span>
              <span class="is-sr-only">Links to Code Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-pwc">Papers with Code</span> <em>(<a href="https://paperswithcode.com/" target="_blank">What is Papers with Code?</a>)</em>
          </div>
        </div>


        <div class="columns is-mobile lab-row">
          <div class="column lab-switch">
            <label class="switch">
              <input
                id="sciencecast-toggle"
                data-script-url="/static/browse/0.3.4/js/sciencecast.js"
                type="checkbox" class="lab-toggle" aria-labelledby="label-for-sciencecast">
              <span class="slider"></span>
              <span class="is-sr-only">ScienceCast Toggle</span>
            </label>
          </div>
          <div class="column lab-name">
            <span id="label-for-sciencecast">ScienceCast</span> <em>(<a href="https://sciencecast.org/welcome" target="_blank">What is ScienceCast?</a>)</em>
          </div>
        </div>

      </div>
      <div id="catalyzex-output" style="display:none"></div>
      <div id="dagshub-output" style="display:none"></div>
      <div id="pwc-output" style="display:none"></div>
      <div id="pwc-data-output" style="display:none"></div>
      <div id="sciencecast-output" style="display:none"></div>
    </div>


      <input type="radio" name="tabs" id="labstabs-demos-input">
      <label for="labstabs-demos-input" id="labstabs-demos-label">Demos</label>
      <div class="tab">
        <h1>Demos</h1>
        <div class="toggle">
          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input
                  id="replicate-toggle"
                  data-script-url="/static/browse/0.3.4/js/replicate.js"
                  type="checkbox" class="lab-toggle" aria-labelledby="label-for-replicate">
                <span class="slider"></span>
                <span class="is-sr-only">Replicate Toggle</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-replicate">Replicate</span> <em>(<a href="https://replicate.com/docs/arxiv/about" target="_blank">What is Replicate?</a>)</em>
            </div>
          </div>
          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input
                  id="spaces-toggle"
                  data-script-url="/static/browse/0.3.4/js/spaces.js"
                  type="checkbox" class="lab-toggle" aria-labelledby="label-for-spaces">
                <span class="slider"></span>
                <span class="is-sr-only">Spaces Toggle</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-spaces">Hugging Face Spaces</span> <em>(<a href="https://huggingface.co/docs/hub/spaces" target="_blank">What is Spaces?</a>)</em>
            </div>
          </div>
          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input
                  id="txyz-toggle"
                  data-script-url="/static/browse/0.3.4/js/txyz.js"
                  type="checkbox" class="lab-toggle" aria-labelledby="label-for-txyz">
                <span class="slider"></span>
                <span class="is-sr-only">Spaces Toggle</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-txyz">TXYZ.AI</span> <em>(<a href="https://txyz.ai" target="_blank">What is TXYZ.AI?</a>)</em>
            </div>
          </div>
        </div>
        <div id="replicate-output"></div>
        <div id="spaces-output"></div>
        <div id="txyz-output"></div>
      </div>
      <input type="radio" name="tabs" id="tabfour">
      <label for="tabfour">Related Papers</label>
      <div class="tab">
        <h1>Recommenders and Search Tools</h1>
        <div class="toggle">
          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input id="influenceflower-toggle"
                data-script-url="/static/browse/0.3.4/js/influenceflower.js"
                type="checkbox" class="lab-toggle" aria-labelledby="label-for-influenceflower">
                <span class="slider"></span>
                <span class="is-sr-only">Link to Influence Flower</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-influenceflower">Influence Flower</span> <em>(<a href="https://influencemap.cmlab.dev/" target="_blank">What are Influence Flowers?</a>)</em>
            </div>
          </div>
          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input id="connectedpapers-toggle" type="checkbox" class="lab-toggle"
                       data-script-url="/static/browse/0.3.4/js/connectedpapers.js"
                       aria-labelledby="label-for-connected-papers" >
                <span class="slider"></span>
                <span class="is-sr-only">Connected Papers Toggle</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-connected-papers">Connected Papers</span> <em>(<a href="https://www.connectedpapers.com/about" target="_blank">What is Connected Papers?</a>)</em>
            </div>
          </div>
          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input id="core-recommender-toggle" type="checkbox" class="lab-toggle" aria-labelledby="label-for-core">
                <span class="slider"></span>
                <span class="is-sr-only">Core recommender toggle</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-core">CORE Recommender</span> <em>(<a href="https://core.ac.uk/services/recommender">What is CORE?</a>)</em>
            </div>
          </div>          <div class="columns is-mobile lab-row">
            <div class="column lab-switch">
              <label class="switch">
                <input id="iarxiv-toggle"
                       type="checkbox"
                       class="lab-toggle"
                       data-script-url="/static/browse/0.3.4/js/iarxiv.js"
                       aria-labelledby="label-for-iarxiv">
                <span class="slider"></span>
                <span class="is-sr-only">IArxiv recommender toggle</span>
              </label>
            </div>
            <div class="column lab-name">
              <span id="label-for-iarxiv">IArxiv Recommender</span>
              <em>(<a href="https://iarxiv.org/about">What is IArxiv?</a>)</em>
            </div>
          </div>
</div>
        <div id="influenceflower-output"></div>
        <div id="influenceflower-output-graph" style="display:none">
          <ul class="flower-tabs">
            <li class="active"><a class="btn tab-btn" onclick="openTab(event, 'tab-author')">Author</a></li>
            <li><a class="btn tab-btn" onclick="openTab(event, 'tab-venue')">Venue</a></li>
            <li><a class="btn tab-btn" onclick="openTab(event, 'tab-inst')">Institution</a></li>
            <li><a class="btn tab-btn" onclick="openTab(event, 'tab-topic')">Topic</a></li>
          </ul>
          <div class="flower-tab-content">
            <div class="tab-flower active" id="tab-author"><svg id="flower-graph-author"></svg></div>
            <div class="tab-flower" id="tab-venue"><svg id="flower-graph-venue"></svg></div>
            <div class="tab-flower" id="tab-inst"><svg id="flower-graph-inst"></svg></div>
            <div class="tab-flower" id="tab-topic"><svg id="flower-graph-topic"></svg></div>
          </div>
        </div>
        <div style="min-height: 15px" id="connectedpapers-output"></div>
        <div id="coreRecommenderOutput"></div>
        <div id="iarxivOutput"></div>
      </div>

      <input type="radio" name="tabs" id="tabfive">
      <label for="tabfive">
        About arXivLabs
      </label>
      <div class="tab">
        <div class="columns">
          <div class="column">
            <h1>arXivLabs: experimental projects with community collaborators</h1>
            <p>arXivLabs is a framework that allows collaborators to develop and share new arXiv features directly on our website.</p>
            <p>Both individuals and organizations that work with arXivLabs have embraced and accepted our values of openness, community, excellence, and user data privacy. arXiv is committed to these values and only works with partners that adhere to them.</p>
            <p>Have an idea for a project that will add value for arXiv's community? <a href="https://info.arxiv.org/labs/index.html"><strong>Learn more about arXivLabs</strong></a>.</p>
          </div>
          <div class="column is-narrow is-full-mobile">
            <p class="icon-labs"><svg xmlns="http://www.w3.org/2000/svg" role="presentation" viewBox="0 0 635.572 811"><path d="M175.6 676v27h-27v-27zm-54 27v27h27v-27zm-27 27v27h27v-27zm396-54v27h-27v-27zm0 27v27h27v-27zm27 27v27h27v-27zm-27-414h27v27h-27zm27 0h27v-27h-27zm27-27h27v-27h-27zm-396 45h-27v-27h27zm-27-54h-27v27h27zm-27-27h-27v27h27z"/><path d="M94.6 730v27h-27v-27zm477 0v27h-27v-27zm-27-495h27v27h-27zm-450 18h-27v-27h27zm477 9h27v27h-27zm-54 495h27v27h-27zm-423 0h27v27h-27zm-54-504h27v27h-27z" fill="#666"/><path d="M67.6 730v27h-27v-27zm54 54v27h-27v-27zm0-108v27h27v-27zm-27 27v27h27v-27zm-81 0v27h27v-27zm585 27v27h-27v-27zm-108-54v27h27v-27zm27 27v27h27v-27zm81 0v27h27v-27zm-54-495h27v27h-27zm-54 108h27v-27h-27zm27-27h27v-27h-27zm0-81h27v-27h-27zm-423 18h-27v-27h27zm54 54h-27v27h27zm-27-27h-27v27h27zm0-81h-27v27h27zm423 612v27h-27v-27zm81-522v27h-27v-27zm-585-9v27h-27v-27z" fill="#999"/><path d="M94.6 784v27h-27v-27zm-27-27v27h27v-27zm-27-54v27h27v-27zm27 0v27h27v-27zm0-27v27h27v-27zm27 0v27h27v-27zm0-27v27h27v-27zm27 0v27h27v-27zm-108 81v27h27v-27zm558 54v27h-27v-27zm-27-27v27h27v-27zm27-54v27h27v-27zm-27 0v27h27v-27zm0-27v27h27v-27zm-27 0v27h27v-27zm0-27v27h27v-27zm-27 0v27h27v-27zm108 81v27h27v-27zm0-495h27v27h-27zm-27 27h27v-27h-27zm-54-27h27v-27h-27zm0 27h27v-27h-27zm-27 0h27v-27h-27zm0 27h27v-27h-27zm-27 0h27v-27h-27zm0 27h27v-27h-27zm81-108h27v-27h-27zm-504 45h-27v-27h27zm27-27h-27v27h27zm54-27h-27v27h27zm0 27h-27v27h27zm27 0h-27v27h27zm0 27h-27v27h27zm27 0h-27v27h27zm0 27h-27v27h27zm-81-108h-27v27h27z" fill="#ccc"/><path d="M598.6 665.1H41.5C-76.5 667 176 280.2 176 280.2h53a46.5 46.5 0 0162.8-56.3 29.2 29.2 0 1128.5 35.9h-1a46.5 46.5 0 01-1.5 20.3l142.5-.1s255.3 387 138.3 385.1zM291 181a29.3 29.3 0 10-29.2-29.3A29.3 29.3 0 00291 181zm65.4-66.8a22.4 22.4 0 10-22.5-22.4 22.4 22.4 0 0022.5 22.4z" fill="#fc0"/><path d="M245.5 172V10h153v162s324 495 198 495h-558c-126 0 207-495 207-495zm126 54h56m-13 72h56m-9 72h56m-20 72h56m-22 72h56m-29 72h56m-457-45c20.8 41.7 87.3 81 160.7 81 72.1 0 142.1-38.2 163.4-81" fill="none" stroke="#000" stroke-miterlimit="10" stroke-width="20"/><path d="M273.3 421.7c0 31-9.8 56.3-21.9 56.3s-21.8-25.2-21.8-56.3 9.8-56.3 21.8-56.3 21.9 25.2 21.9 56.3zm114.4-56.3c-12 0-21.8 25.2-21.8 56.3s9.7 56.3 21.8 56.3 21.9-25.2 21.9-56.3-9.8-56.3-21.9-56.3zM150.1 526.6c-18.2 6.7-27.5 22.9-23.2 30.2s14.8-5.5 33-12.2 37.4-4.9 33-12.2-24.5-12.6-42.8-5.8zm296 5.8c-4.2 7.3 14.9 5.5 33.1 12.2s28.7 19.5 33 12.2-5-23.5-23.2-30.2-38.5-1.5-42.8 5.8z"/></svg></p>
          </div>
        </div>
      </div>

    </div>
</div>
<!-- END LABS AREA -->
  <div class="endorsers">
    <a href="/auth/show-endorsers/2206.13080" class="endorser-who">Which authors of this paper are endorsers?</a> |
    <a id="mathjax_toggle" href="javascript:setMathjaxCookie()">Disable MathJax</a> (<a href="https://info.arxiv.org/help/mathjax.html">What is MathJax?</a>)
    <span class="help" style="font-style: normal; float: right; margin-top: 0; margin-right: 1em;"></span>
  </div>
  <script type="text/javascript" language="javascript">mathjaxToggle();</script>
</div>
      </div>
    </main>

    <footer style="clear: both;">
      <div class="columns is-desktop" role="navigation" aria-label="Secondary" style="margin: -0.75em -0.75em 0.75em -0.75em">
        <!-- Macro-Column 1 -->
        <div class="column" style="padding: 0;">
          <div class="columns">
            <div class="column">
              <ul style="list-style: none; line-height: 2;">
                <li><a href="https://info.arxiv.org/about">About</a></li>
                <li><a href="https://info.arxiv.org/help">Help</a></li>
              </ul>
            </div>
            <div class="column">
              <ul style="list-style: none; line-height: 2;">
                <li>
                  <svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 512 512" class="icon filter-black" role="presentation"><title>contact arXiv</title><desc>Click here to contact arXiv</desc><path d="M502.3 190.8c3.9-3.1 9.7-.2 9.7 4.7V400c0 26.5-21.5 48-48 48H48c-26.5 0-48-21.5-48-48V195.6c0-5 5.7-7.8 9.7-4.7 22.4 17.4 52.1 39.5 154.1 113.6 21.1 15.4 56.7 47.8 92.2 47.6 35.7.3 72-32.8 92.3-47.6 102-74.1 131.6-96.3 154-113.7zM256 320c23.2.4 56.6-29.2 73.4-41.4 132.7-96.3 142.8-104.7 173.4-128.7 5.8-4.5 9.2-11.5 9.2-18.9v-19c0-26.5-21.5-48-48-48H48C21.5 64 0 85.5 0 112v19c0 7.4 3.4 14.3 9.2 18.9 30.6 23.9 40.7 32.4 173.4 128.7 16.8 12.2 50.2 41.8 73.4 41.4z"/></svg>
                  <a href="https://info.arxiv.org/help/contact.html"> Contact</a>
                </li>
                <li>
                  <svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 512 512" class="icon filter-black" role="presentation"><title>subscribe to arXiv mailings</title><desc>Click here to subscribe</desc><path d="M476 3.2L12.5 270.6c-18.1 10.4-15.8 35.6 2.2 43.2L121 358.4l287.3-253.2c5.5-4.9 13.3 2.6 8.6 8.3L176 407v80.5c0 23.6 28.5 32.9 42.5 15.8L282 426l124.6 52.2c14.2 6 30.4-2.9 33-18.2l72-432C515 7.8 493.3-6.8 476 3.2z"/></svg>
                  <a href="https://info.arxiv.org/help/subscribe"> Subscribe</a>
                </li>
              </ul>
            </div>
          </div>
        </div>
        <!-- End Macro-Column 1 -->
        <!-- Macro-Column 2 -->
        <div class="column" style="padding: 0;">
          <div class="columns">
            <div class="column">
              <ul style="list-style: none; line-height: 2;">
                <li><a href="https://info.arxiv.org/help/license/index.html">Copyright</a></li>
                <li><a href="https://info.arxiv.org/help/policies/privacy_policy.html">Privacy Policy</a></li>
              </ul>
            </div>
            <div class="column sorry-app-links">
              <ul style="list-style: none; line-height: 2;">
                <li><a href="https://info.arxiv.org/help/web_accessibility.html">Web Accessibility Assistance</a></li>
                <li>
                  <p class="help">
                    <a class="a11y-main-link" href="https://status.arxiv.org" target="_blank">arXiv Operational Status <svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 256 512" class="icon filter-dark_grey" role="presentation"><path d="M224.3 273l-136 136c-9.4 9.4-24.6 9.4-33.9 0l-22.6-22.6c-9.4-9.4-9.4-24.6 0-33.9l96.4-96.4-96.4-96.4c-9.4-9.4-9.4-24.6 0-33.9L54.3 103c9.4-9.4 24.6-9.4 33.9 0l136 136c9.5 9.4 9.5 24.6.1 34z"/></svg></a><br>
                    Get status notifications via
                    <a class="is-link" href="https://subscribe.sorryapp.com/24846f03/email/new" target="_blank"><svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 512 512" class="icon filter-black" role="presentation"><path d="M502.3 190.8c3.9-3.1 9.7-.2 9.7 4.7V400c0 26.5-21.5 48-48 48H48c-26.5 0-48-21.5-48-48V195.6c0-5 5.7-7.8 9.7-4.7 22.4 17.4 52.1 39.5 154.1 113.6 21.1 15.4 56.7 47.8 92.2 47.6 35.7.3 72-32.8 92.3-47.6 102-74.1 131.6-96.3 154-113.7zM256 320c23.2.4 56.6-29.2 73.4-41.4 132.7-96.3 142.8-104.7 173.4-128.7 5.8-4.5 9.2-11.5 9.2-18.9v-19c0-26.5-21.5-48-48-48H48C21.5 64 0 85.5 0 112v19c0 7.4 3.4 14.3 9.2 18.9 30.6 23.9 40.7 32.4 173.4 128.7 16.8 12.2 50.2 41.8 73.4 41.4z"/></svg>email</a>
                    or <a class="is-link" href="https://subscribe.sorryapp.com/24846f03/slack/new" target="_blank"><svg xmlns="http://www.w3.org/2000/svg" viewBox="0 0 448 512" class="icon filter-black" role="presentation"><path d="M94.12 315.1c0 25.9-21.16 47.06-47.06 47.06S0 341 0 315.1c0-25.9 21.16-47.06 47.06-47.06h47.06v47.06zm23.72 0c0-25.9 21.16-47.06 47.06-47.06s47.06 21.16 47.06 47.06v117.84c0 25.9-21.16 47.06-47.06 47.06s-47.06-21.16-47.06-47.06V315.1zm47.06-188.98c-25.9 0-47.06-21.16-47.06-47.06S139 32 164.9 32s47.06 21.16 47.06 47.06v47.06H164.9zm0 23.72c25.9 0 47.06 21.16 47.06 47.06s-21.16 47.06-47.06 47.06H47.06C21.16 243.96 0 222.8 0 196.9s21.16-47.06 47.06-47.06H164.9zm188.98 47.06c0-25.9 21.16-47.06 47.06-47.06 25.9 0 47.06 21.16 47.06 47.06s-21.16 47.06-47.06 47.06h-47.06V196.9zm-23.72 0c0 25.9-21.16 47.06-47.06 47.06-25.9 0-47.06-21.16-47.06-47.06V79.06c0-25.9 21.16-47.06 47.06-47.06 25.9 0 47.06 21.16 47.06 47.06V196.9zM283.1 385.88c25.9 0 47.06 21.16 47.06 47.06 0 25.9-21.16 47.06-47.06 47.06-25.9 0-47.06-21.16-47.06-47.06v-47.06h47.06zm0-23.72c-25.9 0-47.06-21.16-47.06-47.06 0-25.9 21.16-47.06 47.06-47.06h117.84c25.9 0 47.06 21.16 47.06 47.06 0 25.9-21.16 47.06-47.06 47.06H283.1z"/></svg>slack</a>
                  </p>
                </li>
              </ul>
            </div>
          </div>
        </div> <!-- end MetaColumn 2 -->
        <!-- End Macro-Column 2 -->
      </div>
    </footer>
  </div>

  <script src="/static/base/1.0.1/js/member_acknowledgement.js"></script>

</body>

</html>
